Ideal boundaries of pseudo-Anosov flows and uniform convergence groups, with connections and applications to large scale geometry

Given a general pseudo-Anosov flow in a three manifold, the orbit space of the lifted flow to the universal cover is homeomorphic to an open disk. We compactify this orbit space with an ideal circle boundary. If there are no perfect fits between stable and unstable leaves and the flow is not topologically conjugate to a suspension Anosov flow, we then show: The ideal circle of the orbit space has a natural quotient space which is a sphere and is a dynamical systems ideal boundary for a compactification of the universal cover of the manifold. The main result is that the fundamental group acts on the flow ideal boundary as a uniform convergence group. Using a theorem of Bowditch, this yields a proof that the fundamental group of the manifold is Gromov hyperbolic and it shows that the action of the fundamental group on the flow ideal boundary is conjugate to the action on the Gromov ideal boundary. This implies that pseudo-Anosov flows without perfect fits are quasigeodesic flows and we show that the stable/unstable foliations of these flows are quasi-isometric. Finally we apply these results to foliations: if a foliation is R-covered or with one sided branching in an atoroidal three manifold then the results above imply that the leaves of the foliation in the universal cover extend continuously to the sphere at infinity.

==> serg.tex <==
% Definitions that use @ : 
\catcode`\@=11

% page heading on even pages gives chapter, but on same side of page
% as for odd pages. 


\newcommand{\zz}{\mbox{${\bf Z} \oplus {\bf Z}$}}
\newcommand{\pa}{\mbox{$<_{\alpha}$}}
\newcommand{\mmp}{\mbox{$[-1,1]$}}
\newcommand{\of}{\mbox{$\overline f$}}
\newcommand{\rr}{\mbox{${\cal R}$}}
\newcommand{\cd}{\mbox{${\cal D}$}}
\newcommand{\cp}{\mbox{${\cal P}$}}
\newcommand{\ct}{\mbox{${\cal T}$}}
\newcommand{\pb}{\mbox{$<_{\beta}$}}
\newcommand{\pu}{\mbox{$<_u$}}
\newcommand{\poa}{\mbox{$>_{\alpha}$}}
\newcommand{\pou}{\mbox{$>_u$}}
\newcommand{\oh}{\mbox{$\overline h$}}
\newcommand{\og}{\mbox{$\overline g$}}
\newcommand{\spr}{\mbox{${\bf S}^2 \times {\bf S}^1$}}
\newcommand{\cs}{\mbox{${\bf S}^1$}}
\newcommand{\sss}{\mbox{${\bf S}^2$}}
\newcommand{\ch}{\mbox{$\widehat{\bf C}$}}
\newcommand{\pp}{\mbox{$\Phi_{\theta}$}}
\newcommand{\ii}{\mbox{${\cal I}$}}
\newcommand{\dd}{\mbox{${\cal D}$}}
\newcommand{\ccl}{\mbox{${\cal L}$}}
\newcommand{\kk}{\mbox{${\cal K}$}}
\newcommand{\ca}{\mbox{${\cal A}$}}
\newcommand{\is}{\mbox{${\cal I}^s$}}
\newcommand{\iu}{\mbox{${\cal I}^u$}}
\newcommand{\res}{\mbox{${\cal R}^s$}}
\newcommand{\reu}{\mbox{${\cal R}^u$}}
\newcommand{\bp}{\mbox{$B^+$}}
\newcommand{\bn}{\mbox{$B^-$}}
\newcommand{\ba}{\mbox{${\bf A}$}}
\newcommand{\aaa}{\mbox{${\cal A}$}}
\newcommand{\aap}{\mbox{${\cal A}_1$}}
\newcommand{\bb}{\mbox{${\cal B}$}}
\newcommand{\ak}{\mbox{${\cal A}_{\kappa}$}}
\newcommand{\at}{\mbox{${\cal A}_{\tau}$}}
\newcommand{\otsf}{\mbox{${\overline \tau^s_F}$}}
\newcommand{\otuf}{\mbox{${\overline \tau^u_F}$}}
\newcommand{\ots}{\mbox{${\overline \tau^s}$}}
\newcommand{\otu}{\mbox{${\overline \tau^u}$}}
\newcommand{\ap}{\mbox{${\cal A}_{\alpha}$}}
\newcommand{\ab}{\mbox{${\cal A}_{\beta}$}}
\newcommand{\ag}{\mbox{${\cal A}_g$}}
\newcommand{\lat}{\mbox{${\cal L A}_{\tau}$}}
\newcommand{\lak}{\mbox{${\cal L A}_{\kappa}$}}
\newcommand{\lal}{\mbox{${\cal L A}_{\alpha}$}}
\newcommand{\lag}{\mbox{${\cal L A}_{\gamma}$}}
\newcommand{\lab}{\mbox{${\cal L A}_{\beta}$}}
\newcommand{\la}{\mbox{${\cal L A}$}}
\newcommand{\af}{\mbox{${\cal A}_f$}}
\newcommand{\uu}{\mbox{${\cal U}$}}
\newcommand{\ro}{\mbox{${\cal R}$}}
\newcommand{\vv}{\mbox{${\cal V}$}}
\newcommand{\we}{\mbox{${\cal W}$}}
\newcommand{\re}{\mbox{${\cal R}$}}
\newcommand{\wwx}{\mbox{${\cal WX}$}}
\newcommand{\et}{\mbox{$\eta _-$}}
\newcommand{\tsv}{\mbox{$\sigma ^s_e$}}
\newcommand{\hhu}{\mbox{${\cal H} ^u$}}
\newcommand{\hhs}{\mbox{${\cal H} ^s$}}
\newcommand{\hu}{\mbox{${\cal H}(\widetilde {\cal F} ^u)$}}
\newcommand{\hs}{\mbox{${\cal H}(\widetilde {\cal F} ^s)$}}
\newcommand{\hp}{\mbox{${\cal H}$}}
\newcommand{\tup}{\mbox{$\Theta ^u_+$}}
\newcommand{\tun}{\mbox{$\Theta ^u_-$}}
\newcommand{\tsp}{\mbox{$\Theta ^s_+$}}
\newcommand{\tsn}{\mbox{$\Theta ^s_-$}}
\newcommand{\vs}{\mbox{$\varphi_s$}}
\newcommand{\vu}{\mbox{$\varphi_u$}}
\newcommand{\vg}{\mbox{$\varphi_G$}}
\newcommand{\vf}{\mbox{$\varphi_F$}}
\newcommand{\vif}{\mbox{$\varphi^{\infty}_F$}}
\newcommand{\vig}{\mbox{$\varphi^{\infty}_G$}}
\newcommand{\vil}{\mbox{$\varphi^{\infty}_L$}}
\newcommand{\vi}{\mbox{$\varphi^{\infty}$}}
\newcommand{\vr}{\mbox{$\varphi _s$}}
\newcommand{\vvv}{\mbox{${\cal V}$}}
\newcommand{\hlf}{\mbox{$X^L_F$}}
\newcommand{\hfl}{\mbox{$X^F_L$}}
\newcommand{\zf}{\mbox{$\zeta_F$}}
\newcommand{\zl}{\mbox{$\zeta_L$}}
\newcommand{\pin}{\mbox{$\partial _{\infty}$}}
\newcommand{\cc}{\mbox{$\cal C$}}
\newcommand{\lsf}{\mbox{${\cal L}^s_F$}}
\newcommand{\luf}{\mbox{${\cal L}^u_F$}}
\newcommand{\oo}{\mbox{$\cal O$}}
\newcommand{\oos}{\mbox{${\cal O}^s$}}
\newcommand{\oou}{\mbox{${\cal O}^u$}}
\newcommand{\ooo}{\mbox{$\cal J$}}
\newcommand{\uo}{\mbox{${\cal J}^u$}}
\newcommand{\so}{\mbox{${\cal J}^s$}}
\newcommand{\ou}{\mbox{${\cal J}^u_+$}}
\newcommand{\rrr}{\mbox{$\times {\bf R}$}}
\newcommand{\rrrr}{\mbox{${\bf R}$}}
\newcommand{\rp}{\mbox{$[0,+\infty)$}}
\newcommand{\pn}{\mbox{$\partial N$}}
\newcommand{\mi}{\mbox{$\widetilde M$}}
\newcommand{\wl}{\mbox{$\widetilde \lambda$}}
\newcommand{\ls}{\mbox{$\Lambda^s$}}
\newcommand{\lu}{\mbox{$\Lambda^u$}}
\newcommand{\wgs}{\mbox{$\widetilde \Lambda^s$}}
\newcommand{\wls}{\mbox{$\widetilde \Lambda^s$}}
\newcommand{\wlu}{\mbox{$\widetilde \Lambda^u$}}
\newcommand{\wcl}{\mbox{$\widetilde {\cal L}$}}
\newcommand{\wlsf}{\mbox{$\widetilde \Lambda^s_F$}}
\newcommand{\wluf}{\mbox{$\widetilde \Lambda^u_F$}}
\newcommand{\wlse}{\mbox{$\widetilde \Lambda^s_E$}}
\newcommand{\wlsg}{\mbox{$\widetilde \Lambda^s_G$}}
\newcommand{\wlsfi}{\mbox{$\widetilde \Lambda^s_{F_i}$}}
\newcommand{\wlsl}{\mbox{$\widetilde \Lambda^s_L$}}
\newcommand{\ww}{\mbox{$\widetilde W$}}
\newcommand{\wws}{\mbox{$\widetilde W^s$}}
\newcommand{\wwu}{\mbox{$\widetilde W^u$}}
\newcommand{\ti}{\mbox{$\partial \widetilde T$}}
\newcommand{\ttt}{\mbox{$\widetilde T$}}
\newcommand{\ppn}{\mbox{$\partial _+ N$}}
\newcommand{\lll}{\mbox{$l _{\epsilon}$}}
\newcommand{\iT}{\mbox{$i _{\widetilde T}$}}
\newcommand{\wwp}{\mbox{$\widetilde \Phi$}}
\newcommand{\wwr}{\mbox{$\widetilde \Phi_{\rrrr}$}}
\newcommand{\w}{\mbox{$\widetilde {\partial _+ C}$}}
\newcommand{\pw}{\mbox{$\varphi _{\widetilde T}$}}
\newcommand{\lmun}{\mbox{$\Gamma ^s \cup \Gamma ^u$}}
\newcommand{\gc}{\mbox{${\cal G}$}}
\newcommand{\gsgg}{\mbox{${\cal G}^s_*$}}
\newcommand{\gl}{\mbox{${\cal G}$}}
\newcommand{\gugg}{\mbox{${\cal G}^u_*$}}
\newcommand{\gsg}{\mbox{${\cal G}^s$}}
\newcommand{\gug}{\mbox{${\cal G}^u$}}
\newcommand{\ga}{\mbox{$\Gamma$}}
\newcommand{\gs}{\mbox{$\Gamma ^s$}}
\newcommand{\gu}{\mbox{$\Gamma ^u$}}
\newcommand{\ggs}{\mbox{${\cal F}^s_T$}}
\newcommand{\ggu}{\mbox{${\cal F}^u_T$}}
\newcommand{\gsr}{\mbox{$\Gamma ^s \times {\bf R}$}}
\newcommand{\gur}{\mbox{$\Gamma ^u \times {\bf R}$}}
\newcommand{\se}{\mbox{$S _{\epsilon}$}}
\newcommand{\gus}{\mbox{$\Gamma ^u \downarrow S_{\epsilon}$}}
\newcommand{\vt}{\mbox{$\overline \varphi _{\widetilde T}$}}
%\newcommand{\vvvv}{\mbox{$\varphi _{\widetilde T}$}}
\newcommand{\hh}{\mbox{${\bf H}^2$}}
\newcommand{\hhh}{\mbox{${\bf H}^3$}}
\newcommand{\lmS}{\mbox{$\Gamma ^s \downarrow S$}}
\newcommand{\lmU}{\mbox{$\Gamma ^u \downarrow S$}}
\newcommand{\lms}{\mbox{$\Gamma ^s \downarrow S_{\epsilon}$}}
\newcommand{\lmu}{\mbox{$\Gamma ^u \downarrow S_{\epsilon}$}}
\newcommand{\wall}{\mbox{$L \times \R$}}
\newcommand{\wa}{\mbox{$\widetilde {\alpha}$}}
\newcommand{\wb}{\mbox{$\widetilde {\beta}$}}
\newcommand{\wdd}{\mbox{$\widetilde {\delta}$}}
\newcommand{\lap}{\mbox{$\Gamma ^s \cup \Gamma ^u \cup Q$}}
\newcommand{\tz}{\mbox{$\widetilde T \times \{ 0 \}$}}
\newcommand{\es}{\mbox{${\cal E}^s_F$}}
\newcommand{\eu}{\mbox{${\cal E}^u_F$}}
\newcommand{\wt}{\mbox{$\widetilde T$}}
\newcommand{\wss}{\mbox{$\widetilde S$}}
\newcommand{\rs}{\mbox{$\widetilde \rho(\widetilde S)$}}
\newcommand{\trs}{\mbox{$\Theta(\widetilde \rho(\widetilde S))$}}
\newcommand{\wn}{\mbox{$\widetilde N$}}
\newcommand{\si}{\mbox{$S^2_{\infty}$}}
\newcommand{\su}{\mbox{$S^1_{\infty}$}}
%\newcommand{\sss}{\mbox{$S^s_{\infty}$}}
\newcommand{\sus}{\mbox{$S^u_{\infty}$}}
\newcommand{\s}{\mbox{$S ^1$}}
\newcommand{\fol}{\mbox{$\cal F$}}
\newcommand{\gal}{\mbox{$\cal G$}}
\newcommand{\gp}{\mbox{$\cal G_+$}}
\newcommand{\gm}{\mbox{$\cal G_-$}}
\newcommand{\gn}{\mbox{$\widetilde {\cal G}$}}
\newcommand{\gmn}{\mbox{$\widetilde {\cal G}_-$}}
\newcommand{\gpn}{\mbox{$\widetilde {\cal G}_+$}}
\newcommand{\fn}{\mbox{$\widetilde {\cal F}$}}
\newcommand{\als}{\mbox{${\cal L} ^s$}}
\newcommand{\lss}{\mbox{${\cal L}^s_*$}}
\newcommand{\alu}{\mbox{${\cal L} ^u$}}
\newcommand{\lsd}{\mbox{${\cal L} ^s_d$}}
\newcommand{\lns}{\mbox{$\widetilde {\cal L} ^s$}}
\newcommand{\lnu}{\mbox{$\widetilde {\cal L} ^u$}}
\newcommand{\fs}{\mbox{${\cal F} ^s$}}
\newcommand{\fu}{\mbox{${\cal F} ^u$}}
\newcommand{\fss}{\mbox{${\cal F} ^{ss}$}}
\newcommand{\fuu}{\mbox{${\cal F} ^{uu}$}}
\newcommand{\fuo}{\mbox{${\cal F} ^{uu}_0$}}
\newcommand{\fnss}{\mbox{$\widetilde {\cal F} ^{ss}$}}
\newcommand{\fnuu}{\mbox{$\widetilde {\cal F} ^{uu}$}}
\newcommand{\fns}{\mbox{${\widetilde {\cal F}}^s $}}
\newcommand{\fnso}{\mbox{${\widetilde {\cal F}}^s_{\cal O} $}}
\newcommand{\fnuo}{\mbox{${\widetilde {\cal F}}^u_{\cal O} $}}
\newcommand{\fnsf}{\mbox{${\widetilde {\cal F}}^s_F $}}
\newcommand{\fnsg}{\mbox{${\widetilde {\cal F}}^s_G $}}
\newcommand{\fnuf}{\mbox{${\widetilde {\cal F}}^u_F $}}
\newcommand{\fnu}{\mbox{${\widetilde {\cal F}}^u $}}
\newcommand{\wv}{\mbox{${\overline {\varphi}}$}}
\newcommand{\oxi}{\mbox{${\overline {\xi}}$}}
\newcommand{\wvv}{\mbox{${\varphi}$}}
\newcommand{\fsS}{\mbox{${\cal F} ^s_S$}}
\newcommand{\fsG}{\mbox{${\cal F} ^s_G$}}
\newcommand{\fsE}{\mbox{${\cal F} ^s_E$}}
\newcommand{\fuG}{\mbox{${\cal F} ^u_G$}}
\newcommand{\fuS}{\mbox{${\cal F} ^u_S$}}
\newcommand{\fsT}{\mbox{${\cal F} ^s_T$}}
\newcommand{\fuT}{\mbox{${\cal F} ^u_T$}}
\newcommand{\fSS}{\mbox{$\widetilde{\cal F} ^s_{\cal S}$}}
\newcommand{\fUS}{\mbox{$\widetilde{\cal F} ^u_{\cal S}$}}
\newcommand{\fnuS}{\mbox{$\widetilde {{\cal F}}^u_S $}}
\newcommand{\fnsS}{\mbox{$\widetilde {{\cal F}}^s_S $}}
\newcommand{\ws}{\mbox{$\widetilde  W^s$}}
\newcommand{\wu}{\mbox{$\widetilde  W^u$}}
\newcommand{\hnt}{homotopically non trivial}
\newcommand{\up}{\mbox{${\cal U} _+$}}
\newcommand{\un}{\mbox{${\cal U} _-$}}
\newcommand{\Dp}{\mbox{$\Delta ^+$}}
\newcommand{\Dn}{\mbox{$\Delta ^-$}}
\newcommand{\fg}{\mbox{$\phi _g$}}
\newcommand{\h}{\mbox{$\bf H$}}

 

\def\@evenhead{\rm \leftmark \hfil \thepage}%        Left heading.
\def\chaptermark#1{\markboth {\sc {\ifnum \c@secnumdepth >\m@ne
      \@chapapp\ \thechapter. \ \fi #1}}{}}%

\catcode`\@=12


